FAIL: Analyzing Software Failures from the News Using LLMs

Software failures inform engineering work, standards, regulations. For example, the Log4J vulnerability brought government and industry attention to evaluating and securing software supply chains. Accessing private engineering records is difficult, so failure analyses tend to use information reported by the news media. However, prior works in this direction have relied on manual analysis. That has limited the scale of their analyses. The community lacks automated support to enable such analyses to consider a wide range of news sources and incidents. In this paper, we propose the Failure Analysis Investigation with LLMs (FAIL) system to fill this gap. FAIL collects, analyzes, and summarizes software failures as reported in the news. FAIL groups articles that describe the same incidents. It then analyzes incidents using existing taxonomies for postmortems, faults, and system characteristics. To tune and evaluate FAIL, we followed the methods of prior works by manually analyzing 31 software failures. FAIL achieved an F1 score of 90% for collecting news about software failures, a V-measure of 0.98 for merging articles reporting on the same incident, and extracted 90% of the facts about failures. We then applied FAIL to a total of 137,427 news articles from 11 providers published between 2010 and 2022. FAIL identified and analyzed 2457 distinct failures reported across 4,184 articles. Our findings include: (1) current generation of large language models are capable of identifying news articles that describe failures, and analyzing them according to structured taxonomies; (2) high recurrences of similar failures within organizations and across organizations; and (3) severity of the consequences of software failures have increased over the past decade. The full FAIL database is available so that researchers, engineers, and policymakers can learn from a diversity of software failures.

==> promptengineering.tex <==

\iffalse
\subsection{Prompt Engineering}
Using the training set (n=30) of the manually analyzed sample dataset, we experimented with the prompts used in the pipeline and the parameters of the LLM to improve the performance of the pipeline.

\subsubsection{Prompts} 
~\cref{table: Prompts}
Organize by actions of the pipeline.
Label the kind of task for each prompt.
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}

\begin{table*}[]
\scriptsize
\resizebox{\textwidth}{!}{%
\begin{tabular}{lllp{1.5cm}lp{8cm}}
Cat.                              & Prmt ID & Pip ID & Key                   & Task           & Prompt                                                                                                                                                                                                                                                                                                                                                \\
\multirow{4}{*}{\rotatebox[origin=c]{90}{Tasks   for pipeline}} & 1         & 1           & Describes Failure     & Classify & Does the provided article report on software failure incident(s)?   (software failure could mean a [keywords])                                                                                                                            \\
                                      & 2         & 1           & Analyzable Failure    & Classify & Does the provided article contain enough information about the provided   criteria to conduct a failure analysis of the software failure incident(s)?   Criteria: System that failed, cause of failure, and impact of failure.                                                                                                                        \\
                                      & 3         & 4           & Summary               & Summarize  & Summarize the software failure incident. Include information about when   the failure occured, what system failed, the cause of failure, the impact of   failure, the responsible entity(s), and the impacted entity(s).                                                                                                                              \\
                                      & 4         & 4           & Index                 & Classify & Does the provided paragraph 1 and paragraph 2 describe the same software   failure incident(s)?                                                                                                                                                                                                                                                       \\
\multirow{3}{*}{\rotatebox[origin=c]{90}{Misc   incident info}} & 5         & 6           & Title                 & QA             & Provide a 10 word title for the software failure incident.                                                                                                                                                                                                                                                                                            \\
                                      & 6         & 6           & Summary               & QA             & Summarize the software failure incident. Include information about when   the failure occured, what system failed, the cause of failure, the impact of   failure, the responsible entity(s), and the impacted entity(s).                                                                                                                              \\
                                      & 7         & 6           & Time                  & QA             & When did the software failure incident happen? If possible, calculate   using article published date and relative time mentioned in article.                                                                                                                                                                                                          \\
\multirow{7}{*}{\rotatebox[origin=c]{90}{Postmortem info}}      & 8         & 6           & System                & QA             & What system failed in the software failure incident?                                                                                                                                                                                                                                                                                                  \\
                                      & 9         & 6           & Responsible Org       & QA             & Which entity(s) was responsible for causing the software failure?                                                                                                                                                                                                                                                                                     \\
                                      & 10        & 6           & Impacted Org          & QA             & Which entity(s) was impacted by the software failure?                                                                                                                                                                                                                                                                                                 \\
                                      & 11        & 6           & SE Failure Causes     & QA             & What were the software causes of the failure incident?                                                                                                                                                                                                                                                                                                \\
                                      & 12        & 6           & Non-SE Failure Causes & QA             & What were the non-software causes of the failure incident?                                                                                                                                                                                                                                                                                            \\
                                      & 13        & 6           & Impacts               & QA             & What happened due to the software failure incident?                                                                                                                                                                                                                                                                                                   \\
                                      & 14        & 6           & Mitigations           & QA             & What could have prevented the software failure incident?                                                                                                                                                                                                                                                                                              \\
\multirow{14}{*}{\rotatebox[origin=c]{90}{Taxonomy}}            & 15        & 6           & Phase                 & MCQA           & Was the software failure due to 'system design' (option 0) or 'operation'   (option 1) faults or 'both' (option 2) or 'neither' (option 3) or 'unknown'   (option -1)?                                                                                                                                                                                \\
                                      & 16        & 6           & Boundary              & MCQA           & Was the software failure due to faults from 'within the system' (option   0) or from 'outside the system' (option 1) or 'both' (option 2) or 'neither'   (option 3) or 'unknown' (option -1)?                                                                                                                                                         \\
                                      & 17        & 6           & Nature                & MCQA           & Was the software failure due to 'human actions' (option 0) or 'non human   actions' (option 1) or 'both' (option 2) or 'neither' (option 3) or 'unknown'   (option -1)?                                                                                                                                                                               \\
                                      & 18        & 6           & Dimension             & MCQA           & Was the software failure due to 'hardware' (option 0) or 'software'   (option 1) faults or 'both' (option 2) or 'neither' (option 3) or 'unknown'   (option -1)?                                                                                                                                                                                      \\
                                      & 19        & 6           & Objective             & MCQA           & Was the software failure due to 'malicious' (option 0) or 'non-malicious'   (option 1) faults or 'both' (option 2) or 'neither' (option 3) or 'unknown'   (option -1)?                                                                                                                                                                                \\
                                      & 20        & 6           & Intent                & MCQA           & Was the software failure due to 'deliberate' (option 0) or 'accidental'   (option 1) fault or 'both' (option 2) or 'neither' (option 3) or 'unknown'   (option -1)?                                                                                                                                                                                   \\
                                      & 21        & 6           & Capability            & MCQA           & Was the software failure 'accidental' (option 0) or due to 'development   incompetence' (option 1) or 'both' (option 2) or 'neither' (option 3) or   'unknown' (option -1)?                                                                                                                                                                           \\
                                      & 22        & 6           & Duration              & MCQA           & Was the software failure 'permanent' (option 0) or 'temporary' (option 1)   or 'intermittent' (option 2) or 'unknown' (option -1)?                                                                                                                                                                                                                    \\
                                      & 23        & 6           & Domain                & MCQA           & What application domain is the system: 'automotive' (option 0) or   'critical infrastructure' (option 1) or 'healthcare' (option 2) or 'energy'   (option 3) or 'transportation' (option 4) or 'infrastructure' (option 5) or   'aerospace' (option 6) or 'telecommunications' (option 7) or 'consumer   device' (option 8) or 'unknown' (option -1)? \\
                                      & 24        & 6           & CPS                   & MCQA           & Does the system contain software that controls physical components (cyber   physical system) or is it an IoT system: 'true' (option true) or 'false'   (option false) or 'unknown' (option -1)?                                                                                                                                                       \\
                                      & 25        & 6           & Perception            & MCQA           & Was the software failure due to 'sensors' (option 0) or 'actuators'   (option 1) or 'processing unit' (option 2) or 'network communication' (option   3) or 'embedded software' (option 4) or 'unknown' (option -1)?                                                                                                                                  \\
                                      & 26        & 6           & Communication         & MCQA           & Was there a software failure at the communication level? If false,   (option false). If true, then was the failure at the 'link level' (option 1)   or 'connectivity level' (option 2) or 'unknown' (option -1)?                                                                                                                                      \\
                                      & 27        & 6           & Application           & MCQA           & Was there a software failure at the application level: 'true' (option   true) or 'false' (option false) or 'unknown' (option -1)?                                                                                                                                                                                                                     \\
                                      & 28        & 6           & Behaviour             & MCQA           & Was the software failure due to a 'crash' (option 0) or 'omission'   (option 1) or 'timing' (option 2) or 'value' (option 3) or 'Byzantine' fault   (option 4) or 'unknown' (option -1)?                                                                                                                                                             
\end{tabular}%
}

\caption{Prompts used by the pipeline \TODO{OUTDATED}} \label{table: Prompts}
\end{table*}
\TODO{Remove Pip ID and Task? Reference Prompt ID in the pipeline figure instead?}
\subsubsection{Engineering}
Try Langchain's auto prompt engineering tool: 
\url{https://python.langchain.com/docs/modules/data_connection/retrievers/MultiQueryRetriever}

\subsubsection{Tuning the parameters of ChatGPT}
Discuss how temperature was tuned and its effects and our observations.

\subsubsection{Prompt engineering \TODO{Outdated}} \label{sec:PromptEngineering}
To extract correct and relevant responses using ChatGPT, we had to conduct prompt engineering. 
First, we experimented with the amount of postmortem and taxonomy information that could be gathered reliably within each query. 
We learned that the reliability of the responses improved when the chatbot is given more "space"~\cite{OpenAICookbook2023}.
For instance, when multiple classification questions are asked about the taxonomy of a failure at once, the chatbot changes its answer within its response: \\

\noindent\fbox{\begin{minipage}{26em}
\begin{itemize}
    \item[\iconHuman] {
    1. Was the failure due to 'system design' (option 0) or 'operation' (option 1) faults or \ldots? \\
    2. Was the failure due to faults from 'within the system' (option 0) or from 'outside the system' (option 1) or \ldots? \\
    3. Was the failure due to 'hardware' (option 0) or 'software' (option 1) faults or \ldots? \\
    \ldots}
    \item[\iconChatbot] {
    1. Option 0: \textbf{system design} \\
    2. Option 1: outside the system \\
    3. Option 1: software \\
    \ldots
    \\
    Explanation: \\
    1. The failure was due to an \textbf{operational} fault because \ldots
    }
\end{itemize}
\end{minipage}}


However, when the questions are asked individually, the chatbot's responses are more reliable. 
Additionally, we observed that asking for the rationale for choosing an answer before selecting an answer improves the correctness of a response; consistent with the idea of "thinking out loud" before selecting an answer~\cite{OpenAICookbook2023}


Second, we learned that describing taxonomy terms in queries improved the chatbot's ability to find relevant information from the articles.  
For example, changing the fault boundary terms from `internal' and `external' to `within the system' and `outside the system' improved the responses from the chatbot. 
Furthermore, providing more freedom to choose multiple or none of the taxonomy options improved the chatbot's reliability, since it decrease the rate of miss-classifications.
Additionally, the reliability of taxonomizing unspecified topics in the articles was improved by adding an 'unknown' option to the taxonomy prompts. 

Third, we experimented with the parameters of the chatbot.
We varied the temperature between 0 to 1 to control the randomness and creativity of the model. 
We observed a trade-off between reliability and usefulness. 
With a high temperature, the model was less reliable in taxonomizing categories that were not explicitly discussed in the article, however, the model was effective at leveraging its knowledge to choose options and provide well-thought-out rationales.
With a low temperature, the model was more reliable in the options it chose for taxonomizing a failure, however, it often chose the `unknown' option. 
The rationale that the model provided suggests that it adheres to exactly to the prose in the article, and less on its own knowledge -- minimizing the usefulness of an LLM.

%Shifting article from user content to system content: less focus on the article but better & more reliable responses. \\

Additionally, we constructed prompts to provide responses in a consistent structure. 
We achieved this by specifying options clearly, providing an example response structure, and providing explicit instructions in upper-case letters with restrictive words (\ie only and must). 
\fi


